The Medial Axis of a Multi-Layered Environment and its Application as a Navigation Mesh

Path planning for walking characters in complicated virtual environments is a fundamental task in simulations and games. A navigation mesh is a data structure that allows efficient path planning. The Explicit Corridor Map (ECM) is a navigation mesh based on the medial axis. It enables path planning for disk-shaped characters of any radius. In this paper, we formally extend the medial axis (and therefore the ECM) to 3D environments in which characters are constrained to walkable surfaces. Typical examples of such environments are multi-storey buildings, train stations, and sports stadiums. We give improved definitions of a walkable environment (WE: a description of walkable surfaces in 3D) and a multi-layered environment (MLE: a subdivision of a WE into connected layers). We define the medial axis of such environments based on projected distances on the ground plane. For an MLE with $n$ boundary vertices and $k$ connections, we show that the medial axis has size $O(n)$, and we present an improved algorithm that constructs the medial axis in $O(n \log n \log k)$ time. The medial axis can be annotated with nearest-obstacle information to obtain the ECM navigation mesh. Our implementations show that the ECM can be computed efficiently for large 2D and multi-layered environments, and that it can be used to compute paths within milliseconds. This enables simulations of large virtual crowds of heterogeneous characters in real-time.

==> section-operations.tex <==
\section{Operations} \label{s:operations}

% --- TODO: Replace 5 and 6 by a single section with applications?
This section defines a number of operations on the ECM: cell relations, point location, retraction, and dynamic updates.
These operations are useful for many path planning and crowd simulation algorithms.

\begin{figure*}[htb]
	\centering
	\subfigure[ECM cells \label{fig:u-ecm-cells}]{
		\includegraphics[height=40mm]{fig/u-ecm-cells.pdf}
	}
	\subfigure[Cell relations \label{fig:u-ecm-cellrelations}]{
		\includegraphics[height=40mm]{fig/u-ecm-cellrelations2.pdf}
	}
	\subfigure[Retractions \label{fig:u-retraction}]{
		\includegraphics[height=40mm]{fig/u-ecm-retractions.pdf}
	}
	\caption{
	\NiceSubref{fig:u-ecm-cells} An ECM cell is the polygonal area associated with two subsequent bending points. Some examples of cells have been shaded. 
	\NiceSubref{fig:u-ecm-cellrelations} 
	Cell relations allow us to travel between ECM cells. 
	For instance, \textit{Next} (shown in black) and \textit{Twin} (shown in gray) can be used to follow the ECM cells around an obstacle.
	\NiceSubref{fig:u-retraction} Examples of query points (shown as large dots), their nearest obstacle points (small dots), and their retractions (circles).
	%All points along a dashed line segment have the same retraction.
	}
\end{figure*}

%   =====================================================================================

\subsection{Cells and Adjacency} \label{s:operations:cells}

% ---  TODO: Shorten? May not need its own section.
The ECM partitions the free space \Efree\ into non-overlapping polygonal \emph{cells}.

\begin{defi}[ECM cell]
	An ECM cell $C$ is the obstacle-free polygon associated with two consecutive bending points $bp_1(C)$ and $bp_2(C)$ of an ECM edge.
	The boundary of this cell is given by the positions $p_i$ and the nearest obstacle points $l_i$ and $r_i$ of both bending points.
	In counterclockwise order, the boundary consists of $p_1(C)$, $r_1(C)$, $r_2(C)$, $p_2(C)$, $l_2(C)$, $l_1(C)$, and $p_1(C)$ again (to close the loop).
\end{defi}

\cref{fig:u-ecm-cells} highlights a number of cells in our example ECM.
Note that we now use the indices 1 and 2 to denote the first and second bending point of a cell; these are not related to the indices of the bending points along their ECM edge.
Also, note that some boundary points of a cell can coincide, e.g.\ when a nearest obstacle is a point, or at a degree-1 vertex, 
where the nearest obstacle points coincide with the vertex itself.
An example of the latter is shown in the top-right corner of \cref{fig:u-ecm-cells}.

Recall from \cref{s:2d:ecm} that the ECM is an undirected graph and that every edge can be specified in two directions.
Consequently, there are also two ways to define a cell.
Whenever the direction of an edge is relevant, we speak of \emph{directed cells}, which are unique.
For directed cells, we can define adjacency relations as in a doubly-connected edge list.
%One can think of these relations as pointers from one cell to another.
These relations are useful in many geometric operations on the ECM, such as visibility queries and dynamic updates.

\begin{defi}[Next cell]
For a directed ECM cell $C$, the \emph{next cell} \NextCell{C} is the directed cell that continues along the same obstacle as $C$ on the left side.
\begin{enumerate}
	\item If $C$ does not lie at the end of an ECM edge, then \NextCell{C} is the next directed cell along the same edge.
	\item If $C$ lies at the end of an ECM edge and the end vertex $v$ has other outgoing edges, then \NextCell{C} is the first directed cell of the next clockwise edge from $v$.
	\item If $C$ lies at the end of an ECM edge and the end vertex $v$ has degree 1, then $\NextCell{C} = \nil$.
\end{enumerate}
\end{defi}

We define the \emph{previous cell} \PrevCell{C} reversely.
The third relation is the \emph{twin} relation:

\begin{defi}[Twin cell]
For a directed ECM cell $C$, the \emph{twin cell} \TwinCell{C} is the directed cell that describes the same area in the opposite direction.
\end{defi}

By combining the \textit{Next}, \textit{Prev}, and \textit{Twin} relations, we can move between all cells in a connected component of the ECM.
\cref{fig:u-ecm-cellrelations} shows an example of how the relations can be used to trace all ECM cells around an obstacle. 

\begin{comment}
\cref{fig:u-ecm-cellrelations} shows the cell relations in our example environment.
One can think of these relations as \emph{pointers} from one cell to another.
In our own implementation, we do not store the relations explicitly; instead, we find a next, previous, or twin cell on the fly when needed.
If the ECM can change at run-time due to dynamic updates (see \cref{s:operations:dynamic}), this on-the-fly approach is more practical than maintaining pointers.
The operations typically still run in constant time because each vertex has a constant degree (except in degenerate cases).
\end{comment}

%   =====================================================================================

\subsection{Point Location and Retraction} \label{s:operations:pointlocation}

% --- TODO: Move to Section 3 or 6?
Since the ECM cells are non-overlapping, we can easily perform a \emph{point location} query to find out in which ECM cell a query point in \Efree\ is located.
If a query point lies on the border between cells, we accept any of these cells as a valid answer.
Note that we only need the ECM \emph{cells} (which are all polygonal) and not their corresponding medial axis arcs (which may be parabolic arcs).

For an environment of complexity $n$, there are \BigO{n} cells of constant complexity.
Point location queries can be answered in \BigO{\log n} time using e.g.\ a trapezoidal map, which can be built in \BigO{n \log n} time \cite{deBerg2008-CompGeom}.
For multi-layered environments, we create a separate data structure for each layer. 
A query point in an MLE is specified by a 2D point and a layer ID, such that we can simply perform 2D point location within the specified layer.

Once the cell containing a query point $p$ has been determined, we can compute the \emph{nearest obstacle point} $np(p)$ in constant time because each cell has constant complexity.
Hence, in a crowd simulation application, we can easily determine how far each character is removed from the nearest boundary.

Points in the free space can also be \emph{retracted} onto the medial axis.
In robot motion planning, the term `retraction' is used for a function that maps points in \Efree\ onto the medial axis \cite{Wilmarth1999-Retraction},
as well as for complete planning methods based on this principle \cite{ODunlaing1985-Retraction}.
We use the following definition:

\begin{defi}[Retraction]
For any point $p$ in the free space \Efree, the \emph{retraction} \Retraction{p} is a unique projection of $p$ onto the medial axis.
\begin{enumerate}
	\item If $p$ lies on the medial axis, then $\Retraction{p} = p$.
	\item If $p$ does not lie on the medial axis, let $l$ be the half-line that starts at $np(p)$ and passes through $p$.
	\Retraction{p} is the first intersection of $l$ with the medial axis.
\end{enumerate}
\end{defi}

\cref{fig:u-retraction} shows examples of retractions. 
Observe that \Retraction{p} always lies in the same ECM cell as $p$ 
because the half-line $l$ is defined such that the nearest obstacle does not change along $l$ before intersecting the medial axis.
Therefore, a retraction is easy to compute using the ECM: it can be found in \BigO{\log n} time by using a point location query followed by constant-time geometric operations.
\cref{s:pathplanning} will show how retractions can be used for path planning queries.

%   =====================================================================================

\subsection{Dynamic Updates} \label{s:operations:dynamic}

In modern computer games and simulations, the geometry of the environment can change at runtime.
For example, a bridge can collapse, an alley can be blocked by a parked vehicle, or a new route can appear when a wall is destroyed.
Path planning and crowd simulation in such \emph{dynamic environments} have become increasingly important.
Consequently, it is desirable for navigation meshes to support fast local updates in response to dynamic events.
A character can then efficiently plan a new optimal path in the updated mesh by re-using parts of its previous path \cite{vanToll2015-Replanning}.

In previous work \cite{vanToll2012-Dynamic}, we have presented algorithms that update the Explicit Corridor Map locally due to the insertion or deletion of an obstacle $P$.
Using these algorithms, the ECM can adapt to dynamic events in real-time.
The algorithms assume that $P$ does not touch or intersect any other geometry.

When inserting $P$, we construct the loop of new ECM edges around $P$ based on an incremental construction algorithm for Voronoi diagrams \cite{Green1978-IncrementalVoronoi}.
This takes \BigO{m + \log n} time, where $m$ is the combined complexity of the neighboring obstacles for $P$. 
The \BigO{\log n} factor is due to an initial point location query.

When deleting $P$, we locally repair the ECM in the area that used to have $P$ as a nearest obstacle \cite{Devillers1999-VoronoiDeletion}. 
This can be performed in \BigO{m \log m + \log n} time by recomputing the medial axis for the neighboring obstacles of $P$.
The \BigO{\log n} factor can be removed if $P$ already has a pointer to one of its medial axis edges.
It is likely that other algorithms \cite{Aggarwal1989-LinearVoronoi,Khramtcova2015-LinearDeletion} can be used to improve the running time to \BigO{m}. 
However, it is currently unclear to what extent these algorithms are applicable to multi-layered environments. 
We will not explore this further in this paper.

==> section-pathplanning.tex <==
\section{Path Planning and Crowd Simulation} \label{s:pathplanning}

In this section, we show how to use the ECM navigation mesh for path planning and crowd simulation applications.

\begin{figure*}[t]
	\centering
	\subfigure[Initial query \label{fig:u-pathplanning-query}]{
		\includegraphics[height=40mm]{fig/u-pathplanning-query.pdf}
	}
	\subfigure[Corridor \label{fig:u-pathplanning-corridor}]{
		\includegraphics[height=40mm]{fig/u-pathplanning-corridor.pdf}
	}
	\subfigure[Routes with clearance \label{fig:u-pathplanning-routes}]{
		\includegraphics[height=40mm]{fig/u-pathplanning-routes.pdf}
	}
	\caption{Path planning in the ECM.
	\NiceSubref{fig:u-pathplanning-query} Given two positions $s$ and $g$, the retraction method is used to compute a path from $s$ to $g$ along the medial axis.
	\NiceSubref{fig:u-pathplanning-corridor} A corridor describes the free space around the medial axis path.
	\NiceSubref{fig:u-pathplanning-routes} Within the corridor, 
	we can compute indicative routes (shown as bold curves)	such as shortest routes with varying amounts of preferred clearance.
	}
\end{figure*}

%   =====================================================================================

\subsection{Multi-Level Crowd Simulation} \label{s:pathplanning:multilevel}

We have recently proposed a general framework for efficiently simulating crowds of heterogeneous characters with individual preferences and goals \cite{vanToll2015-Framework}.
This framework consists of five levels: high-level planning, global route planning, route following, local movement, and animation.
A navigation mesh is useful for the middle three levels, which concern the \emph{geometric} aspects of planning.

\begin{comment}
This framework consists of five levels, as shown in \cref{fig:planning-levels}.
We refer the reader to the original publication for a detailed description of the framework.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.6\textwidth]{fig/planning-levels.pdf}
	\caption{Outline of a multi-level crowd simulation framework, as described in previous work \cite{vanToll2015-Framework}. 
	The five levels of planning are shown on the left.
	A navigation mesh is useful for global route planning, route following, and local movement.
	\label{fig:planning-levels}}
\end{figure}

A navigation mesh is useful for the \emph{geometric} aspects of planning: global route planning, route following, and local movement.
\end{comment}
The goal of global route planning is to compute an \emph{indicative route} for a character, which is a rough indication of the path to traverse.
In each simulation step, the route following level computes a \emph{preferred velocity} for the character, 
which is a speed and direction that smoothly advances the character along the indicative route. 
The local movement level converts this preferred velocity to a velocity that attempts to avoid (future) collisions with other characters in the simulation.
%The local movement level then converts this preferred velocity to an \emph{actual velocity}: a speed and direction that is similar to the character's preference while avoiding (future) collisions with other characters in the simulation.

Path following and local movement are beyond the scope of this paper, 
but it is worth noting that the ECM's efficient geometric operations (point location, retraction, and computing nearest obstacles) 
are important for making the multi-level simulation run in real-time.
We will now show how to perform global route planning using the ECM.

\subsection{Global Path Planning in the ECM} \label{s:pathplanning:ecm}

Even though navigation meshes consist of 2D regions, global path planning is almost always performed using an abstract graph representation.
The \emph{dual graph} of a navigation mesh is obtained by assigning one vertex to each mesh region, and adding an edge between each pair of vertices for which the regions are adjacent.

The ECM is different from other meshes in this aspect: 
it is already an explicit graph (namely the medial axis) and it is annotated with extra information to subdivide the environment into cells.
This means that global path planning can immediately be performed on the medial axis itself.
Global planning is efficient because the medial axis is a sparse graph.
Furthermore, thanks to the clearance information in each ECM bending point, 
we can easily compute the \emph{minimum clearance} along an edge in a pre-processing step.
This enables path planning for disk-shaped characters of any radius. 
The concepts in this subsection apply to both 2D and multi-layered environments.

\subsubsection{Computing an ECM Path} \label{s:pathplanning-corridor}

The first step of computing an indicative route in the ECM is computing a valid path on the medial axis.
This is equivalent to the \emph{retraction method} for motion planning \cite{ODunlaing1985-Retraction}.
Given a start position $s$ and a goal position $g$ in \Efree, we first compute their retractions, 
and then we compute an optimal path on the medial axis from \Retraction{s} to \Retraction{g} using the A* search algorithm, 
while ignoring edges along which the minimum clearance is too small for the character to pass through.
\cref{fig:u-pathplanning-query} shows an example of a medial axis path between two query points.
It is common to use distance-based costs to obtain \emph{shortest} paths, but one could also compute optimal paths based on other criteria, 
e.g.\ the expected walking time based on crowd density information \cite{vanToll2012-Density}.

The result of a path planning query on the ECM is a sequence of medial axis edges and their annotations.
The collision-free space around this path can be described using a \emph{corridor}, 
which is the sequence of ECM cells along the path combined with the maximum-clearance disks at its ECM vertices \cite{Geraerts2010-ECM}.
\cref{fig:u-pathplanning-corridor} shows an example of a corridor.

\subsubsection{Computing an Indicative Route} \label{s:pathplanning:indicativeroutes}

An ECM path can be converted into various types of indicative routes in \BigO{m} time, where $m$ is the number of ECM cells along the path \cite{Geraerts2010-ECM}.
We can use a funnel algorithm to obtain the \emph{shortest path} within a corridor, while keeping a preferred distance to obstacles whenever possible.
Whenever this preferred amount of clearance is not available, the indicative route follows the medial axis.
Examples are displayed in \cref{fig:u-pathplanning-routes}.
It is also easy to compute indicative routes that stay on the left or right side of the free space (or any interpolation of these extremes) using the boundaries of ECM cells.
Varying the `side preference' among characters in a simulation is a convenient way to obtain diversity in the crowd.
